Testing and Estimating Structural Breaks in Time Series and Panel Data in Stata

Identifying structural change is a crucial step in analysis of time series and panel data. The longer the time span, the higher the likelihood that the model parameters have changed as a result of major disruptive events, such as the 2007--2008 financial crisis and the 2020 COVID--19 outbreak. Detecting the existence of breaks, and dating them is therefore necessary, not only for estimation purposes but also for understanding drivers of change and their effect on relationships. This article introduces a new community contributed command called xtbreak, which provides researchers with a complete toolbox for analysing multiple structural breaks in time series and panel data. xtbreak can detect the existence of breaks, determine their number and location, and provide break date confidence intervals. The new command is used to explore changes in the relationship between COVID--19 cases and deaths in the US, using both aggregate and state level data, and in the relationship between approval ratings and consumer confidence, using a panel of eight countries.

==> StataOutput/EX1_ts_TestH3s.log.tex <==
. xtbreak test d.deaths d.L(1/3).cases , hypothesis(3) breaks(5) sequential vce(hac)
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)              81.12             6.09            4.66            4.03
 F(2|1)              76.03             6.59            5.24            4.64
 F(3|2)              76.72             6.92            5.61            4.99
 F(4|3)              76.01             7.33            5.87            5.23
 F(5|4)             464.49             7.49            6.05            5.45
\HLI{80}
Detected number of breaks:                5               5               5
\HLI{80}
The detected number of breaks indicates the highest number of
 breaks for which the null hypothesis is rejected.
Trimming: 0.15
{\smallskip}


==> StataOutput/EX1_ts_TestH3sbonly.log.tex <==
. xtbreak test d.deaths  , breakconstant nobreakvar(L(1/3).cases)
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)               8.54            12.29            8.58            7.04
 F(2|1)               9.83            13.89           10.13            8.51
 F(3|2)              12.22            14.80           11.14            9.41
 F(4|3)               9.93            15.28           11.83           10.04
 F(5|4)              12.23            15.76           12.25           10.58
\HLI{80}
Detected number of breaks: (min)          .               3               3
                           (max)          .               3               5
\HLI{80}
Null hypothesis rejected more than once after non-rejection.
 The detected number of breaks indicates the minimum and maximum
 number of breaks for which the null hypothesis is rejected.
Trimming: 0.15
{\smallskip}


==> StataOutput/EX1_ts_TestH3sbreakconst.log.tex <==
. xtbreak test d.deaths d.L(1/3).cases , breakconstant
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)              21.88             5.06            4.05            3.56
 F(2|1)               5.30             5.49            4.53            4.03
 F(3|2)              13.05             5.70            4.73            4.33
 F(4|3)               8.93             5.76            4.91            4.50
 F(5|4)              10.53             5.94            5.05            4.61
\HLI{80}
Detected number of breaks: (min)          1               5               5
                           (max)          5               5               5
\HLI{80}
Null hypothesis rejected more than once after non-rejection.
 The detected number of breaks indicates the minimum and maximum
 number of breaks for which the null hypothesis is rejected.
Trimming: 0.15
{\smallskip}


==> StataOutput/EX1_ts_estbreak2.log.tex <==
. xtbreak estimate d.deaths d.L(1/3).cases , breaks(2) 
{\smallskip}
Estimation of break points
                                            Number of obs       =     79
                                            SSR                 =     49.07
                                            Trimming            =      0.15
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        15      2020w22                       2020w21        2020w23
  2        45      2020w52                       2020w51        2021w1 
\HLI{80}


==> StataOutput/EX1_ts_ssr.log.tex <==
. xtbreak est d.deaths d.L(1/3).cases , breaks(1)
{\smallskip}
Estimation of break points
                                                           T    =     79
                                                           SSR  =     60.79
                                                      Trimming  =      0.15
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        16      2020w23                       2020w22        2020w24
\HLI{80}
{\smallskip}
. estat ssr , xlabel(`=yw(2020,1)' "2020"  `=yw(2020,23)' `"" "w23"' `=yw(2021,1)' "2021" `=yw(2021,34)' `"" "w34"' )  scheme(sj) name(ss
> r, replace)
{\smallskip}


==> StataOutput/EX1_xt_estat.log.tex <==
. qui xtreg d.deaths `r(varlist)', fe
{\smallskip}
. qui eststo xtreg: nlcom (regime1: _b[LD_cases1] +  _b[L2D_cases1] + _b[L3D_cases1])  ///
>  (regime2: _b[LD_cases2] +  _b[L2D_cases2] + _b[L3D_cases2]) ///
>  (regime3: _b[LD_cases3] +  _b[L2D_cases3] + _b[L3D_cases3]) ///
>  (regime4: _b[LD_cases4] +  _b[L2D_cases4] + _b[L3D_cases4]) /// 
>  (regime5: _b[LD_cases5] +  _b[L2D_cases5] + _b[L3D_cases5]),  post
{\smallskip}


==> StataOutput/EX1_xt_estimate.log.tex <==
. xtbreak estimate d.deaths d.L(1/3).cases,  breaks(4) trim(0.1) vce(hc)
{\smallskip}
Estimation of break points
                                                           N    =     60
                                                           T    =     79
                                                           SSR  =     13.88
                                                      Trimming  =      0.10
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        7       2020w14                       2020w13        2020w15
  2        14      2020w21                       2020w20        2020w22
  3        46      2021w1                        2020w52        2021w2 
  4        53      2021w8                        2021w7         2021w9 
\HLI{80}


==> StataOutput/EX1_xt_estimate_b4.log.tex <==
. xtbreak estimate d.deaths d.L(1/3).cases, csa(d.l.cases) breaks(4) trim(0.1) vce(wpn)
{\smallskip}
Estimation of break points
                                                           N    =     60
                                                           T    =     79
                                                           SSR  =     10.89
                                                      Trimming  =      0.10
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        7       2020w14                       2020w13        2020w15
  2        14      2020w21                       2020w20        2020w22
  3        45      2020w52                       2020w51        2021w1 
  4        53      2021w8                        2021w7         2021w9 
\HLI{80}
Cross-section averages:
  with breaks: LD.cases


==> StataOutput/EX1_xt_general.log.tex <==
. xtbreak d.deaths d.L(1/3).cases, vce(hc)
{\smallskip}
Test for multiple breaks at unknown breakdates
(Ditzen, Karavias \& Westerlund. 2024)
H0: no break(s) vs. H1: 1 <= s <= 5 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 UDmax               11.90             6.09            4.74            4.13
\HLI{80}
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)              11.90             6.09            4.66            4.03
 F(2|1)               9.31             6.59            5.24            4.64
 F(3|2)               6.66             6.92            5.61            4.99
 F(4|3)               4.72             7.33            5.87            5.23
 F(5|4)               4.97             7.49            6.05            5.45
\HLI{80}
Detected number of breaks:                2               3               3
\HLI{80}
The detected number of breaks indicates the highest number of
 breaks for which the null hypothesis is rejected.
{\smallskip}
Estimation of break points
                                            Number of obs       =   4740
                                            Number of Groups    =     60
                                            Obs per group       =     79
                                            SSR                 =     18.04
                                            Trimming            =      0.15
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        12      2020w19                       2020w16        2020w22
  2        36      2020w43                       2020w42        2020w44
  3        47      2021w2                        2021w1         2021w3 
\HLI{80}


==> StataOutput/EX1_xt_table_b3_b4.tex <==
Regime 1     &       0.133   &       0.133   \\
            &     (0.004)***&     (0.024)***\\
Regime 2     &       0.056   &       0.056   \\
            &     (0.003)***&     (0.016)***\\
Regime 3(a)     &       0.015   &       0.018   \\
            &     (0.000)***&     (0.002)***\\
Regime 3b    &               &       0.014   \\
            &               &     (0.002)***\\
Regime 4     &       0.010   &       0.010   \\
            &     (0.000)***&     (0.002)***\\
Regime 5     &       0.011   &       0.011   \\
            &     (0.001)***&     (0.001)***\\


==> StataOutput/EX1_xt_testH1.log.tex <==
. xtbreak test d.deaths d.L(1/3).cases, h(1) breaks(1)  csa(d.L(1/3).cases)
Test for multiple breaks at known breakdates
(Karavias, Narayan \& Westerlund. 2021)
H0: no break(s) vs. H1: 1 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 supF                66.39             6.09            4.66            4.03
\HLI{80}
Estimated break points: 2020w20
Trimming: 0.15
Cross-section averages:
  with breaks: LD.cases L2D.cases L3D.cases


==> StataOutput/EX1_xt_testH12.log.tex <==
. xtbreak test d.deaths d.L(1/3).cases, h(1) breaks(5)  csa(d.L(1/3).cases)
{\smallskip}
Test for multiple breaks at unknown breakdates
(Ditzen, Karavias \& Westerlund. 2021)
H0: no break(s) vs. H1: 5 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 supF                28.77             2.90            2.49            2.30
\HLI{80}
Estimated break points: 2020w18 2020w29 2020w43 2021w2 2021w13
Trimming: 0.15
Cross-section averages:
  with breaks: LD.cases L2D.cases L3D.cases


==> StataOutput/EX1_xt_testH2.log.tex <==
. xtbreak test d.deaths d.L(1/3).cases, h(2) breaks(5)  csa(d.L(1/3).cases)
{\smallskip}
Test for multiple breaks at unknown breakdates
(Ditzen, Karavias \& Westerlund. 2024)
H0: no break(s) vs. H1: 1 <= s <= 5 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 UDmax               66.39             6.09            4.74            4.13
\HLI{80}
Trimming: 0.15
Cross-section averages:
  with breaks: LD.cases L2D.cases L3D.cases


==> StataOutput/EX2_Emp2_tab.log.tex <==
. * Col 1)
. xtbreak  d.approval d.CCI , trim(0.05)  strict python
{\smallskip}
Test for multiple breaks at unknown breakdates
(Ditzen, Karavias \& Westerlund. 2024)
H0: no break(s) vs. H1: 1 <= s <= 19 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 UDmax(tau)          15.60            13.74           10.17            8.78
\HLI{80}
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)              15.60            13.58            9.63            8.02
 F(2|1)              22.25            15.03           11.14            9.56
 F(3|2)               5.29            15.62           12.16           10.45
\HLI{80}
Detected number of breaks:                2               2               2
\HLI{80}
The detected number of breaks indicates the highest number of
 breaks for which the null hypothesis is rejected.
{\smallskip}
Estimation of break points
                                            Number of obs       =   3064
                                            Number of Groups    =      8
                                            Obs per group       =    383
                                            SSR                 =  35364.86
                                            Trimming            =      0.05
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        344     2018m9                        2017m3         2020m3 
  2        363     2020m4                        2018m10        2021m10
\HLI{80}
{\smallskip}
. 
. * Col 2)
. xtbreak  d.approval d.CCI , trim(0.05) vce(hc) strict python
{\smallskip}
Test for multiple breaks at unknown breakdates
(Ditzen, Karavias \& Westerlund. 2024)
H0: no break(s) vs. H1: 1 <= s <= 19 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 UDmax(tau)           9.73            13.74           10.17            8.78
\HLI{80}
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)               9.73            13.58            9.63            8.02
 F(2|1)              14.24            15.03           11.14            9.56
 F(3|2)               2.30            15.62           12.16           10.45
\HLI{80}
Detected number of breaks:                .               2               2
\HLI{80}
The detected number of breaks indicates the highest number of
 breaks for which the null hypothesis is rejected.
{\smallskip}
Estimation of break points
                                            Number of obs       =   3064
                                            Number of Groups    =      8
                                            Obs per group       =    383
                                            SSR                 =  35364.86
                                            Trimming            =      0.05
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        344     2018m9                        2017m3         2020m3 
  2        363     2020m4                        2018m10        2021m10
\HLI{80}
{\smallskip}
. 
. * Col 3)
. xtbreak  d.approval d.CCI , trim(0.05) nobreakvar(ElectionQ) strict python
{\smallskip}
Test for multiple breaks at unknown breakdates
(Ditzen, Karavias \& Westerlund. 2024)
H0: no break(s) vs. H1: 1 <= s <= 19 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 UDmax(tau)          13.91            13.74           10.17            8.78
\HLI{80}
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)              12.63            13.58            9.63            8.02
 F(2|1)              26.99            15.03           11.14            9.56
 F(3|2)               5.32            15.62           12.16           10.45
\HLI{80}
Detected number of breaks:                2               2               2
\HLI{80}
The detected number of breaks indicates the highest number of
 breaks for which the null hypothesis is rejected.
{\smallskip}
Estimation of break points
                                            Number of obs       =   3064
                                            Number of Groups    =      8
                                            Obs per group       =    383
                                            SSR                 =  34584.14
                                            Trimming            =      0.05
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        344     2018m9                        2017m3         2020m3 
  2        363     2020m4                        2019m2         2021m6 
\HLI{80}
{\smallskip}
. 
. * Col 4)
. xtbreak  d.approval d.CCI , trim(0.05) nobreakvar(ElectionQ) nofixedeffects strict python
{\smallskip}
Test for multiple breaks at unknown breakdates
(Ditzen, Karavias \& Westerlund. 2024)
H0: no break(s) vs. H1: 1 <= s <= 19 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 UDmax(tau)          13.85            13.74           10.17            8.78
\HLI{80}
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)              12.51            13.58            9.63            8.02
 F(2|1)              26.97            15.03           11.14            9.56
 F(3|2)               6.98            15.62           12.16           10.45
\HLI{80}
Detected number of breaks:                2               2               2
\HLI{80}
The detected number of breaks indicates the highest number of
 breaks for which the null hypothesis is rejected.
{\smallskip}
Estimation of break points
                                            Number of obs       =   3064
                                            Number of Groups    =      8
                                            Obs per group       =    383
                                            SSR                 =  34773.36
                                            Trimming            =      0.05
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        344     2018m9                        2017m3         2020m3 
  2        363     2020m4                        2019m2         2021m6 
\HLI{80}
{\smallskip}
. 
. * Col 5)
. xtbreak  d.approval d.CCI , trim(0.05) nobreakvar(ElectionQ) nofixedeffects breakconstant cvalue(0.90) strict python
{\smallskip}
Test for multiple breaks at unknown breakdates
(Ditzen, Karavias \& Westerlund. 2024)
H0: no break(s) vs. H1: 1 <= s <= 19 break(s)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 UDmax(tau)           8.13             8.39            6.63            5.84
\HLI{80}
{\smallskip}
Sequential test for multiple breaks at unknown breakpoints
(Ditzen, Karavias \& Westerlund. 2024)
{\smallskip}
                \HLI{17} Bai \& Perron Critical Values \HLI{17}
                     Test          1\% Critical     5\% Critical    10\% Critical
                  Statistic          Value            Value           Value
\HLI{80}
 F(1|0)               6.56             8.32            6.45            5.51
 F(2|1)              19.80             8.99            7.25            6.39
 F(3|2)               4.00             9.33            7.71            6.86
\HLI{80}
Detected number of breaks:                2               2               2
\HLI{80}
The detected number of breaks indicates the highest number of
 breaks for which the null hypothesis is rejected.
{\smallskip}
Estimation of break points
                                            Number of obs       =   3064
                                            Number of Groups    =      8
                                            Obs per group       =    383
                                            SSR                 =  34716.10
                                            Trimming            =      0.05
\HLI{80}
  \#      Index     Date                          [95\% Conf. Interval]
\HLI{80}
  1        344     2018m9                        2018m6         2018m12
  2        363     2020m4                        2020m2         2020m6 
\HLI{80}

